Exploring Proxying QUIC and HTTP/3 for Satellite Communication

Low-Earth Orbit satellites have gained momentum to provide Internet connectivity, augmenting those in the long-established geostationary orbits. At the same time, QUIC has been developed as the new transport protocol for the web. While QUIC traffic is fully encrypted, intermediaries such as performance enhancing proxies (PEPs) - in the past essential for Internet over satellite performance - can no longer tamper with and optimize transport connections. In this paper, we present a satellite emulation testbed and use it to compare QUIC and TCP as well as HTTP/3 and HTTP/1.1 with and without minimal PEP functionality. Evaluating goodput over time, we find that the slow start threshold is reached up to 2s faster for QUIC PEP in comparison to QUIC Non-PEP. Moreover, we find that HTTP/3 and HTTP/3-PEP outperform HTTP/1.1 and HTTP/1.1-PEP in multiple web performance scenarios, where HTTP/3-PEP improves over HTTP/3 for Page Load Time by over 7s in edge cases. Hence, our findings hint that these performance gains may warrant exploring PEPs for QUIC.

==> figures/starlink.rtt.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=0.5\linewidth,trim=0 0 0 0, clip]{figures/sat-1st-hop-rtt.pdf}
	\caption{Distribution of $\sim$305k first hop RTT measurements performed over a period of 96 hours using the Starlink LEO constellation.\todo{update figure}
	} %[]{}
	\label{fig:starlink.rtt}
\end{figure}

